MCQUIC: Multicast and unicast in a single transport protocol

Multicast enables efficient one-to-many communications. Several applications benefit from its scalability properties, e.g., live-streaming and large-scale software updates. Historically, multicast applications have used specialized transport protocols. The flexibility of the recently standardized QUIC protocol opens the possibility of providing both unicast and multicast services to applications with a single transport protocol. We present MCQUIC, an extended version of the QUIC protocol that supports multicast communications. We show how QUIC features and built-in security can be leveraged for multicast transport. We present the design of MCQUIC and implement it in Cloudflare quiche. We assess its performance through benchmarks and in emulated networks under realistic scenarios. We also demonstrate MCQUIC in a campus network. By coupling QUIC with our multicast extension, applications can rely on multicast for efficiency with the possibility to fall back on unicast in case of incompatible network conditions.

==> sections/related-work.tex <==
In their paper, Perkins \emph{et al.}~\cite{perkins2018real} outline the need of real-time applications to support low-latency communication, and propose QUIC-R, a minimal set of extensions in QUIC for that support. Even tough this is not directly related to multicast, QUIC-R also extends QUIC to support low-latency applications. Moreover, the authors highlight that \longn{} may be beneficial in that context.

HTTP over multicast QUIC~\cite{pardue-quic-http-mcast-11} is an IETF draft designing HTTP communication over QUIC leveraging an IP multicast network. The multicast behavior (such as channel discovery, channel join) is implemented within HTTP. Our work focuses on implementing multicast inside QUIC while keeping unicast QUIC untouched. Our design allows to support \emph{multicast as a service}, i.e., that a multicast client can fall back on its unicast session with the source in case they cannot meet the channel requirements. The draft also suggests using Forward Erasure Correction to recover lost packets and suggest the use of digital signatures to authenticate payload. However, we could not find any public implementation of this draft fulfilling its specifications. Our design comes with a working implementation showing the feasibility of the approach. We deeply analyze the reliability mechanism and suggest multiple authenticity schemes with performance benchmarks.

Multicast extensions for QUIC~\cite{jholland-quic-multicast-02} is another IETF draft. This document specifies extensions inside QUIC to support multicast delivery. The design presented in this paper follows some guidelines from the draft: the \texttt{MC\_ANNOUNCE}, \texttt{MC\_KEY} and \texttt{MC\_STATE} of \shortn{} have similar behavior than this IETF document. However, our design suggest a more scalable approach to an increased number of receivers. First, lost packets are recovered with Forward Erasure Correction frames that are sent on the multicast channel. On the other hand, the draft~\cite{jholland-quic-multicast-02} suggests to retransmit lost frames using the unicast session between the server and the client. Second, we suggest multiple approaches to solve the source authentication problem, discussed in Section~\ref{sec:authentication}. The \emph{asymmetric signature} and \emph{stream-level asymmetric signature} methods propose schemes independent of the number of clients in the multicast group. Multicast extensions for QUIC~\cite{jholland-quic-multicast-02} recommend a different approach where data packets sent on the multicast channels are authenticated by hasing them and sending them either individually on each client or on another multicast channel whose packets carrying these hashed are also authenticated using the same authentication mechanism. Such approach, at some point, requires packet hashes to be regularly sent on the unicast session of each client of the multicast group, which is not be scalable for large multicast groups. It introduces a linear dependency between the number of recipients and the amount of bytes being sent, which is against the multicast philosophy. We believe that our approach is more scalable both for the recovery and authentication mechanism, and the benchmarks presented in Section~\ref{sec:reliability} and Section~\ref{sec:authentication} show that the induced overhead remains reasonable. 
Finally, our approach leverages multipath QUIC~\cite{ietf-quic-multipath-04} to implement multicast, which renders the communication on the clients more straightforward as the multicast channel is considered as a second path with a different cryptographic context.
Again, no recent open source implementation of this draft is available for direct comparison with our implementation.
